Gaia Data Release 3: Gaia scan-angle dependent signals and spurious periods

Context: Gaia DR3 time series data may contain spurious signals related to the time-dependent scan angle. Aims: We aim to explain the origin of scan-angle dependent signals and how they can lead to spurious periods, provide statistics to identify them in the data, and suggest how to deal with them in Gaia DR3 data and in future releases. Methods: Using real Gaia data, alongside numerical and analytical models, we visualise and explain the features observed in the data. Results: We demonstrated with Gaia data that source structure (multiplicity or extendedness) or pollution from close-by bright objects can cause biases in the image parameter determination from which photometric, astrometric and (indirectly) radial velocity time series are derived. These biases are a function of the time-dependent scan direction of the instrument and thus can introduce scan-angle dependent signals, which in turn can result in specific spurious periodic signals. Numerical simulations qualitatively reproduce the general structure observed in the spurious period and spatial distribution of photometry and astrometry. A variety of statistics allows for identification of affected sources. Conclusions: The origin of the scan-angle dependent signals and subsequent spurious periods is well-understood and is in majority caused by fixed-orientation optical pairs with separation <0.5" (amongst which binaries with P>>5y) and (cores of) distant galaxies. Though the majority of sources with affected derived parameters have been filtered out from the Gaia archive, there remain Gaia DR3 data that should be treated with care (e.g. gaia_source was untouched). Finally, the various statistics discussed in the paper can not only be used to identify and filter affected sources, but alternatively reveal new information about them not available through other means, especially in terms of binarity on sub-arcsecond scale.

==> acronyms.tex <==
\section{Acronyms}\label{sec:acronyms}
{\small
\begin{tabular}{ll}
\hline\hline
\textbf{Acronym}  &  \textbf{Description}  \\ 
%2MASS & Two-Micron All Sky Survey \\
ADQL&Astronomical Data Query Language \\
%AGB&Asymptotic Giant Branch (star) \\
AL & ALong scan (direction) \\
AC & ACross scan (direction) \\
AF & Astrometric Field (instrument) \\
AGIS & Astrometric Global Iterative Solution \\
%AP & Astrophysical Parameters \\
%BH & Black hole \\
BP & Gaia Blue Photometer \\
CCD & Charge-Coupled Device \\
%CMD & Colour Magnitude Diagram \\
%DoF&Degree(s) of Freedom \\
DPAC & Data Processing and Analysis Consortium \\
DR1 & \gaia Data Release 1 \\
DR2 & \gaia Data Release 2 \\
DR3 & \gaia Data Release 3 \\
DR4 & \gaia Data Release 4 \\
%EB&Eclipsing Binary \\
EDR3 & Gaia Early Data Release 3 \\
EPSL & Ecliptic Pole Scanning Law \\
EO & Extended Objects (Gaia DPAC pipeline) \\
%FLAME & Final Luminosity Age Mass Estimator \\
FAP & False Alarm Probability \\
FoV & Field of View \\
%FWHM&Full Width at Half-Maximum \\
%GALEX&GALaxy Evolution eXplorer \\
GAPS & Gaia Andromeda Photometric Survey \\
GoF & Goodness of Fit \\
GOST & Gaia Observation Forecast Tool \\
%GSPPhot&Generalised Stellar Parametriser PHOTometry \\
%GSPSpec&Generalised Stellar Parametriser SPECtroscopy \\
%GUCD & Gaia Ultra-cool Dwarf\\
%HealPix & Hierarchical Equal Area isoLatitude Pixelisation \\
%HPM & High Proper Motion \\
%HRD & Hertzsprung-Russell diagram\\
IDU & Intermediate Data Updating \\
IPD & Image Parameter Determination \\
%IMF&Initial Mass Function \\
%LMC&Large Magellanic Cloud \\
%LPV & Long Period Variables \\
LSF & Line Spread Function (one dimensional) \\
%MAD & Median Absolute Deviation \\
%MS&Main Sequence (star) \\
%NLS & Non linear spectro \\
%NS & Neutron star \\
NCP & North Celestial Pole \\
NEP & North Ecliptic Pole \\
NSL & Nominal Scanning Law \\
NSS & Non-Single Star \\
%PMa&proper motion anomaly \\
PSF & Point Spread Function (two dimensional) \\
%RGB&Red Giant Branch (star) \\
%RMS&Root-Mean-Square \\
RP & Gaia Red Photometer \\
%RUWE&Re-normalised unit-weight error \\
RV & Radial Velocity \\
RVS&Radial Velocity Spectrometer (instrument) \\
SB & Spectroscopic Binary  \\
SB1&Single-lined Spectroscopic Binary \\
SB2&Double-lined Spectroscopic Binary \\
SEAPipe & Source Environment Analysis pipeline \\
SEP & South Ecliptic Pole \\
SM & Sky Mapper (instrument) \\
%SNR & Signal to Noise ratio (also denoted SN and S/N)\\
%TBO & Two body orbits \\
%UCD&Ultra cool dwarf (star) \\
%UV&UltraViolet \\
%VIMF & variable-induced movers fixed \\
%WD & White dwarf\\
\hline
\end{tabular} 
}
